Perceptual adjustment queries and an inverted measurement paradigm for low-rank metric learning

We introduce a new type of query mechanism for collecting human feedback, called the perceptual adjustment query ( PAQ). Being both informative and cognitively lightweight, the PAQ adopts an inverted measurement scheme, and combines advantages from both cardinal and ordinal queries. We showcase the PAQ in the metric learning problem, where we collect PAQ measurements to learn an unknown Mahalanobis distance. This gives rise to a high-dimensional, low-rank matrix estimation problem to which standard matrix estimators cannot be applied. Consequently, we develop a two-stage estimator for metric learning from PAQs, and provide sample complexity guarantees for this estimator. We present numerical simulations demonstrating the performance of the estimator and its notable properties.

==> sections/bib.tex <==
\begin{thebibliography}{10}

\bibitem{agrawal2018rewriting}
Akshay Agrawal, Robin Verschueren, Steven Diamond, and Stephen Boyd.
\newblock A rewriting system for convex optimization problems.
\newblock {\em Journal of Control and Decision}, 5(1):42--60, 2018.

\bibitem{bao2013moments}
Yong Bao and Raymond Kan.
\newblock On the moments of ratios of quadratic forms in normal random
  variables.
\newblock {\em Journal of Multivariate Analysis}, 117:229--245, 2013.

\bibitem{barnett2003modern}
William Barnett.
\newblock The modern theory of consumer behavior: Ordinal or cardinal?
\newblock {\em The Quarterly Journal of Austrian Economics}, 6(1):41--65, 2003.

\bibitem{batley2008ordinal}
Richard Batley.
\newblock On ordinal utility, cardinal utility and random utility.
\newblock {\em Theory and Decision}, 64:37--63, 2008.

\bibitem{bellet2015robustness}
Aur{\'e}lien Bellet and Amaury Habrard.
\newblock Robustness and generalization for metric learning.
\newblock {\em Neurocomputing}, 151:259--267, 2015.

\bibitem{bellet2022metric}
Aur{\'e}lien Bellet, Amaury Habrard, and Marc Sebban.
\newblock {\em Metric Learning}.
\newblock Springer Nature, 2022.

\bibitem{bian2012constrained}
Wei Bian and Dacheng Tao.
\newblock Constrained empirical risk minimization framework for distance metric
  learning.
\newblock {\em IEEE Transactions on Neural Networks and Learning Systems},
  23(8):1194--1205, 2012.

\bibitem{boucheron2013concentration}
St{\'e}phane Boucheron, G{\'a}bor Lugosi, and Pascal Massart.
\newblock {\em Concentration Inequalities: A Nonasymptotic Theory of
  Independence}.
\newblock Oxford University Press, 2013.

\bibitem{cai2013sparse}
T~Tony Cai and Anru Zhang.
\newblock Sparse representation of a polytope and recovery of sparse signals
  and low-rank matrices.
\newblock {\em IEEE Transactions on Information Theory}, 60(1):122--132, 2013.

\bibitem{cai2015rop}
T~Tony Cai and Anru Zhang.
\newblock Rop: Matrix recovery via rank-one projections.
\newblock {\em The Annals of Statistics}, 43(1):102--138, 2015.

\bibitem{canal2020tuplewise}
Gregory Canal, Stefano Fenu, and Christopher Rozell.
\newblock Active ordinal querying for tuplewise similarity learning.
\newblock In {\em Proceedings of the AAAI Conference on Artificial
  Intelligence}, volume~34, 2020.

\bibitem{canal2022one}
Gregory Canal, Blake Mason, Ramya Korlakai~Vinayak, and Robert Nowak.
\newblock One for all: Simultaneous metric and preference learning over
  multiple users.
\newblock In {\em Advances in Neural Information Processing Systems},
  volume~35, 2022.

\bibitem{candes2011tight}
Emmanuel~J Candes and Yaniv Plan.
\newblock Tight oracle inequalities for low-rank matrix recovery from a minimal
  number of noisy random measurements.
\newblock {\em IEEE Transactions on Information Theory}, 57(4):2342--2359,
  2011.

\bibitem{chandrasekher2022alternating}
Kabir~Aladin Chandrasekher, Mengqi Lou, and Ashwin Pananjady.
\newblock Alternating minimization for generalized rank one matrix sensing:
  Sharp predictions from a random initialization.
\newblock {\em arXiv preprint arXiv:2207.09660}, 2022.

\bibitem{chen2015exact}
Yuxin Chen, Yuejie Chi, and Andrea~J Goldsmith.
\newblock Exact and stable covariance estimation from quadratic sampling via
  convex programming.
\newblock {\em IEEE Transactions on Information Theory}, 61(7):4034--4059,
  2015.

\bibitem{davenport2016overview}
Mark~A Davenport and Justin Romberg.
\newblock An overview of low-rank matrix recovery from incomplete observations.
\newblock {\em IEEE Journal of Selected Topics in Signal Processing},
  10(4):608--622, 2016.

\bibitem{diamond2016cvxpy}
Steven Diamond and Stephen Boyd.
\newblock {CVXPY}: {A} {P}ython-embedded modeling language for convex
  optimization.
\newblock {\em Journal of Machine Learning Research}, 17(83):1--5, 2016.

\bibitem{fan2017estimation}
Jianqing Fan, Quefeng Li, and Yuyan Wang.
\newblock Estimation of high dimensional mean regression in the absence of
  symmetry and light tail assumptions.
\newblock {\em {Journal of the Royal Statistical Society Series B, Statistical
  methodology}}, 79(1):247--265, 2016.

\bibitem{fan2021shrinkage}
Jianqing Fan, Weichen Wang, and Ziwei Zhu.
\newblock A shrinkage principle for heavy-tailed data: High-dimensional robust
  low-rank matrix recovery.
\newblock {\em The Annals of Statistics}, 49(3):1239--1266, 2021.

\bibitem{goffin2011relative}
Richard~D. Goffin and James~M. Olson.
\newblock Is it all relative? {C}omparative judgments and the possible
  improvement of self-ratings and ratings of others.
\newblock {\em Perspectives on Psychological Science}, 6(1):48--60, 2011.

\bibitem{goodfellow2014generative}
Ian Goodfellow, Jean Pouget-Abadie, Mehdi Mirza, Bing Xu, David Warde-Farley,
  Sherjil Ozair, Aaron Courville, and Yoshua Bengio.
\newblock Generative adversarial nets.
\newblock {\em Advances in Neural Information Processing Systems (NeurIPS)},
  27, 2014.

\bibitem{griffin2008calibration}
Dale Griffin and Lyle Brenner.
\newblock {\em Perspectives on Probability Judgment Calibration}, chapter~9.
\newblock Wiley-Blackwell, 2008.

\bibitem{guo2014guaranteed}
Zheng-Chu Guo and Yiming Ying.
\newblock Guaranteed classification via regularized similarity learning.
\newblock {\em Neural Computation}, 26(3):497--522, 2014.

\bibitem{harik2009generalizability}
Polina Harik, Brian Clauser, Irina Grabovsky, Ronald Nungester, David Swanson,
  and Ratna Nandakumar.
\newblock An examination of rater drift within a generalizability theory
  framework.
\newblock {\em Journal of Educational Measurement}, 46:43--58, 2009.

\bibitem{harkonen2020ganspace}
Erik H{\"a}rk{\"o}nen, Aaron Hertzmann, Jaakko Lehtinen, and Sylvain Paris.
\newblock {GANSpace}: Discovering interpretable {GAN} controls.
\newblock {\em Advances in Neural Information Processing Systems}, 33, 2020.

\bibitem{harzing2009national}
Anne-Wil Harzing, Joyce Baldueza, Wilhelm Barner-Rasmussen, Cordula Barzantny,
  Anne Canabal, Anabella Davila, Alvaro Espejo, Rita Ferreira, Axele Giroud,
  Kathrin Koester, Yung-Kuei Liang, Audra Mockaitis, Michael~J. Morley, Barbara
  Myloni, Joseph~O.T. Odusanya, Sharon~Leiba O'Sullivan, Ananda~Kumar
  Palaniappan, Paulo Prochno, Srabani~Roy Choudhury, Ayse Saka-Helmhout,
  Sununta Siengthai, Linda Viswat, Ayda~Uzuncarsili Soydas, and Lena Zander.
\newblock Rating versus ranking: What is the best way to reduce response and
  language bias in cross-national research?
\newblock {\em International Business Review}, 18(4):417--432, 2009.

\bibitem{hsu2016loss}
Daniel Hsu and Sivan Sabato.
\newblock Loss minimization and parameter estimation with heavy tails.
\newblock {\em Journal of Machine Learning Research}, 17(1):543--582, 2016.

\bibitem{karras2020analyzing}
Tero Karras, Samuli Laine, Miika Aittala, Janne Hellsten, Jaakko Lehtinen, and
  Timo Aila.
\newblock Analyzing and improving the image quality of stylegan.
\newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition (CVPR)}, pages 8110--8119, 2020.

\bibitem{kueng2017low}
Richard Kueng, Holger Rauhut, and Ulrich Terstiege.
\newblock Low rank matrix recovery from rank one measurements.
\newblock {\em Applied and Computational Harmonic Analysis}, 42(1):88--116,
  2017.

\bibitem{loh2017statistical}
Po-Ling Loh.
\newblock Statistical consistency and asymptotic normality for high-dimensional
  robust {$M$}-estimators.
\newblock {\em The Annals of Statistics}, 45(2):866--896, 2017.

\bibitem{mason2017learning}
Blake Mason, Lalit Jain, and Robert Nowak.
\newblock Learning low-dimensional metrics.
\newblock In {\em Advances in Neural Information Processing Systems},
  volume~30, 2017.

\bibitem{massimino2021you}
Andrew~K Massimino and Mark~A Davenport.
\newblock As you like it: Localization via paired comparisons.
\newblock {\em Journal of Machine Learning Research}, 22(1):8357--8395, 2021.

\bibitem{mcrae2022optimal}
Andrew~D McRae, Justin Romberg, and Mark~A Davenport.
\newblock Optimal convex lifted sparse phase retrieval and {PCA} with an atomic
  matrix norm regularizer.
\newblock {\em IEEE Transactions on Information Theory}, 69(3):1866--1882,
  2022.

\bibitem{mendelson2015learning}
Shahar Mendelson.
\newblock Learning without concentration.
\newblock {\em Journal of the ACM (JACM)}, 62(3):1--25, 2015.

\bibitem{minsker2015geometric}
Stanislav Minsker.
\newblock {Geometric median and robust estimation in Banach spaces}.
\newblock {\em Bernoulli}, 21(4):2308--2335, 2015.

\bibitem{myford2009drift}
Carol~M. Myford and Edward~W. Wolfe.
\newblock Monitoring rater performance over time: A framework for detecting
  differential accuracy and differential scale category use.
\newblock {\em Journal of Educational Measurement}, 46(4):371--389, 2009.

\bibitem{negahban2011estimation}
Sahand Negahban and Martin~J Wainwright.
\newblock Estimation of (near) low-rank matrices with noise and
  high-dimensional scaling.
\newblock {\em The Annals of Statistics}, 39(2):1069--1097, 2011.

\bibitem{negahban2012restricted}
Sahand Negahban and Martin~J Wainwright.
\newblock Restricted strong convexity and weighted matrix completion: Optimal
  bounds with noise.
\newblock {\em Journal of Machine Learning Research}, 13(1):1665--1697, 2012.

\bibitem{negahban2012unified}
Sahand~N Negahban, Pradeep Ravikumar, Martin~J Wainwright, and Bin Yu.
\newblock A unified framework for high-dimensional analysis of ${M}$-estimators
  with decomposable regularizers.
\newblock {\em Statistical Science}, 27(4):538--557, 2012.

\bibitem{nemirovskij1983problem}
Arkadij~Semenovi{\v{c}} Nemirovskij and David~Borisovich Yudin.
\newblock {\em Problem complexity and method efficiency in optimization}.
\newblock Wiley-Interscience, 1983.

\bibitem{raman2014grading}
Karthik Raman and Thorsten Joachims.
\newblock Methods for ordinal peer grading.
\newblock In {\em Proceedings of the ACM SIGKDD International Conference on
  Knowledge Discovery and Data Mining}, volume~20, 2014.

\bibitem{rankin1980system}
William~L. Rankin and Joel~W. Grube.
\newblock A comparison of ranking and rating procedures for value system
  measurement.
\newblock {\em European Journal of Social Psychology}, 10(3):233--246, 1980.

\bibitem{recht2010guaranteed}
Benjamin Recht, Maryam Fazel, and Pablo~A Parrilo.
\newblock Guaranteed minimum-rank solutions of linear matrix equations via
  nuclear norm minimization.
\newblock {\em SIAM review}, 52(3):471--501, 2010.

\bibitem{rudelson2013hanson}
Mark Rudelson and Roman Vershynin.
\newblock Hanson--{W}right inequality and sub-gaussian concentration.
\newblock {\em Electronic Communications in Probability}, 18:1--9, 2013.

\bibitem{shah2016topology}
Nihar~B. Shah, Sivaraman Balakrishnan, Joseph Bradley, Abhay Parekh, Kannan
  Ramchandran, and Martin~J. Wainwright.
\newblock Estimation from pairwise comparisons: Sharp minimax bounds with
  topology dependence.
\newblock {\em Journal of Machine Learning Research}, 17(58):1--47, 2016.

\bibitem{shah2013case}
Nihar~B. Shah, Joseph~K Bradley, Abhay Parekh, Martin Wainwright, and Kannan
  Ramchandran.
\newblock A case for ordinal peer-evaluation in {MOOC}s.
\newblock In {\em NIPS Workshop on Data Driven Education}, 2013.

\bibitem{tropp2015convex}
Joel~A Tropp.
\newblock Convex recovery of a structured signal from independent random linear
  measurements.
\newblock {\em Sampling Theory, a Renaissance: Compressive Sensing and Other
  Developments}, pages 67--101, 2015.

\bibitem{tsybakov2011estimation}
A~Tsybakov and A~Rohde.
\newblock Estimation of high-dimensional low-rank matrices.
\newblock {\em The Annals of Statistics}, 39(2):887--930, 2011.

\bibitem{vershynin2010introduction}
Roman Vershynin.
\newblock Introduction to the non-asymptotic analysis of random matrices.
\newblock {\em arXiv preprint arXiv:1011.3027}, 2010.

\bibitem{vershynin2018high}
Roman Vershynin.
\newblock {\em High-dimensional probability: An introduction with applications
  in data science}, volume~47.
\newblock Cambridge university press, 2018.

\bibitem{wang2019miscalibration}
Jingyan Wang and Nihar~B. Shah.
\newblock Your 2 is my 1, your 3 is my 9: Handling arbitrary miscalibrations in
  ratings.
\newblock In {\em Proceedings of the 18th International Conference on
  Autonomous Agents and Multiagent Systems}, 2019.

\bibitem{xu2020simultaneous}
Austin Xu and Mark Davenport.
\newblock Simultaneous preference and metric learning from paired comparisons.
\newblock {\em Advances in Neural Information Processing Systems}, 33, 2020.

\bibitem{yannakakis2011reporting}
Georgios~N. Yannakakis and John Hallam.
\newblock Ranking vs. preference: A comparative study of self-reporting.
\newblock In Sidney D'Mello, Arthur Graesser, Bj{\"o}rn Schuller, and
  Jean-Claude Martin, editors, {\em Affective Computing and Intelligent
  Interaction}, pages 437--446, Berlin, Heidelberg, 2011. Springer Berlin
  Heidelberg.

\bibitem{ying2009sparse}
Yiming Ying, Kaizhu Huang, and Colin Campbell.
\newblock Sparse metric learning via smooth optimization.
\newblock {\em Advances in Neural Information Processing Systems}, 22, 2009.

\end{thebibliography}
